Fast Iterative Graph Computing with Updated Neighbor States

Enhancing the efficiency of iterative computation on graphs has garnered considerable attention in both industry and academia. Nonetheless, the majority of efforts focus on expediting iterative computation by minimizing the running time per iteration step, ignoring the optimization of the number of iteration rounds, which is a crucial aspect of iterative computation. We experimentally verified the correlation between the vertex processing order and the number of iterative rounds, thus making it possible to reduce the number of execution rounds for iterative computation. In this paper, we propose a graph reordering method, GoGraph, which can construct a well-formed vertex processing order effectively reducing the number of iteration rounds and, consequently, accelerating iterative computation. Before delving into GoGraph, a metric function is introduced to quantify the efficiency of vertex processing order in accelerating iterative computation. This metric reflects the quality of the processing order by counting the number of edges whose source precedes the destination. GoGraph employs a divide-and-conquer mindset to establish the vertex processing order by maximizing the value of the metric function. Our experimental results show that GoGraph outperforms current state-of-the-art reordering algorithms by 1.83x on average (up to 3.34x) in runtime.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> otherfile/sec1-intro.tex <==
\section{Introduction}\label{sec:introduction}
Graph analysis has been widely used %become ubiquitous 
in many fields, such as social recommendation systems~\cite{fan2019graph,wu2018socialgcn}, fraud detection systems~\cite{kurshan2020graph,sarma2020bank}, and infectious disease spread detection and prevention~\cite{ahmed2020covid,bhapkar2020virus}. 
% 先说迭代计算是分析和处理图数据的一种重要手段，比如pr，sssp。
% iteratively performs a relaxation operation on each edge to gradually estimate the shortest distance of each vertex to the source vertex.}
% The vast amount of data generated in production and daily life has led to the creation of large-scale graphs with up to 4.2 billion vertices and 1.7 billion edges\cite{OGB-LSC} \gsf{which kind of graph?}. However, analyzing these large graphs presents a performance bottleneck due to the enormous computations and message-passing process during iterations, as vertices are accessed and computed repeatedly, and messages are transmitted along the edges until the entire graph state converges. 
% \eat{Iterative computation in graph processing, which includes local computation within individual vertices and message passing between vertices, can become computationally intensive when analyzing large-scale graphs due to the repeated access and computation of vertices and message passing along edges until the graph converges.}
The proliferation of data from production and daily activities has resulted in the emergence of large-scale graphs. 
As the size of the graph increases, the analysis overhead increases exponentially. Moreover, most graph computing tasks use complex iterative methods to compute and update the graph states, such as PageRank\cite{page1999pagerank} and Single Source Shortest Path (SSSP), which makes it difficult to improve graph processing efficiency. To effectively process large-scale graph data iteratively, some distributed graph processing systems have
been developed, like Pergel\cite{malewicz2010pregel}, GraphLab\cite{low2014graphlab}, PowerGraph\cite{gonzalez2012powergraph}, Gemini\cite{zhu2016gemini}, Grape\cite{fan2017grape}, PrIter\cite{zhang2011priter}, Maiter\cite{zhang2013maiter}, Ingress\cite{gong2021automating}, just to name a few.
% However, these graph processing systems are primarily concerned with worker coordination for more efficient processing of large-scale graphs distributively, e.g., reducing the communication between workers\cite{gonzalez2012powergraph,chen2019powerlyra,dathathri2018gluon}, reducing the waiting time between workers\cite{zhu2016gemini,zhang2013maiter,xie2015sync}, or reducing redundant stale computation between workers \cite{fan2018adaptive}, without taking into account the computational efficiency of each worker.%这些图处理系统专注于并行和分布式环境下处理大规模数据中的优化，忽略了每台机器的计算效率。

Distributed iterative graph computation includes local computation within each worker for processing its subgraph, and coordination among workers for delivering vertex states or messages between vertices in different workers. 
Previous systems focuses on worker coordination to improve the efficiency of distributed processing of large-scale graphs. This includes reducing worker communication \cite{gonzalez2012powergraph,chen2019powerlyra,dathathri2018gluon}, minimizing waiting time between workers \cite{zhu2016gemini,zhang2013maiter,xie2015sync,fan2018adaptive}, and balancing the load on each worker\cite{vldb19topox}.
% \eat{avoiding redundant computation \cite{fan2018adaptive}.} 
However, these systems typically fail to consider the computational efficiency of individual workers. 
In this paper, we mainly focus on enhancing the performance of graph processing systems by improving the efficiency of each worker. This work starts from the following two observations.


\eat{
\begin{figure}[t]
% \captionsetup{justification=centering}
%\vspace{-0.3in}
   \centering
   %\begin{minipage}{1.55\textwidth}
  \subfloat[Number of iterations]{\includegraphics[width = 0.22\textwidth]{Expr/sec-1/sk-2005_step.pdf}\label{fig:distri_sssp}}\hspace{0.1in}
   \subfloat[Runtime]{\includegraphics[width = 0.22\textwidth]{Expr/sec-1/sk-2005_time.pdf}\label{fig:distri_pagerank}}\hspace{0.05in}
  %\newline
   %\end{minipage}
   %\vspace{-0.15in}
    \caption{\justifying The number of iterations and runtime of PageRank for different graph processing orders on the Indochina and sk-2005, in which the processing orders are yielded by different graph reordering methods. \textit{Original} means the raw graph without reordering. \textit{GoGraph} is the graph reordering method proposed in this paper. To eliminate the influence of coordination between workers, the experiment is performed with a single thread on a PC.}\label{fig:reorder-method}
%\vspace{-0.2in}
\end{figure}
}



\begin{figure}[tbp]
%\vspace{-0.2in} %修改和文章的间距
    \centering
    \subfloat[Graph]{\includegraphics[width=0.2\linewidth]{Figures/pr-iter-1.pdf}\label{fig:pr-eg-1}} 
    \hspace{2mm}
    \subfloat[Processing order 1: $a-b-c-d$]{\includegraphics[width=0.35\linewidth]{Figures/pr-iter-2.pdf}\label{fig:pr-eg-2}} 
    \hspace{2mm}
    \subfloat[Processing order 2: $d-c-b-a$]{\includegraphics[width=0.35\linewidth]{Figures/pr-iter-3.pdf}\label{fig:pr-eg-3}} 
    \caption{The change of vertices state and the number of iterations when performing PageRank with different graph processing orders.}
    \label{fig:pr-iter-eg}
\vspace{0in} %修改和文章的间距
\end{figure}





\begin{table*}[t]
\renewcommand{\arraystretch}{1.2}
\captionsetup{justification=centering}
  \caption{The number of iterations and the total number of cache misses \\ when performing PageRank on the original graph and a reordered graph.}
  \label{tab:factor}
  \centering
  % Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|c|cc|cc|cc|}
\hline
\multirow{2}{*}{} & \multicolumn{2}{c|}{indochaina} & \multicolumn{2}{c|}{sk-2005} & \multicolumn{2}{c|}{cit-patents} \\ \cline{2-7} 
 & \multicolumn{1}{c|}{Origin} & Reorder & \multicolumn{1}{c|}{Origin} & Reorder & \multicolumn{1}{c|}{Origin} & Reorder \\ \hline
Iter. round & \multicolumn{1}{c|}{91} & 61 & \multicolumn{1}{c|}{94} & 70 & \multicolumn{1}{c|}{105} & 91 \\ \hline
Cache miss & \multicolumn{1}{c|}{237,842} & 240,093 & \multicolumn{1}{c|}{995,604} & 1,365,868 & \multicolumn{1}{c|}{930,797,324} & 1,117,899,700 \\ \hline
%Cache miss rate & \multicolumn{1}{c|}{14.60\%} & 17.82\% & \multicolumn{1}{c|}{7.02\%} & 10.51\% & \multicolumn{1}{c|}{58.46\%} & 63.79\% \\ \hline
\end{tabular}
    
\end{table*}





% We found that \gsf{\{the flow of Intro, please see comment\}}%我们发现在每台机器中，不同的顶点处理顺序影响迭代的效率，如图（画个图，pagerank和sssp，三个数据集，三四中reorder方法包括我们的）。然后解释产生这个现象的原因，用一个特别简单的图就行。
\stitle{Observation 1.} We find that the processing order of vertices will reduce or increase the iteration rounds required, thereby affecting the overall computational efficiency.
Take PageRank as an example, as shown in  Figure \ref{fig:pr-iter-eg}, a sample graph is given in Figure  \ref{fig:pr-eg-1}, Figure \ref{fig:pr-eg-2} and Figure \ref{fig:pr-eg-3} list the states (PageRank values) of vertices after the first three iterations and the total rounds of iteration for different processing orders.
% \eat{We found that the processing order of vertices will reduce or increase the iteration rounds required as demonstrated in Figure \ref{fig:pr-iter-eg}, thereby affecting the efficiency of iterative computations.}
%Figure \ref{fig:reorder-method}, we report the number of iterations and runtime of PageRank for different vertex processing orders on the Indochina and sk-2005 datasets. The results show that employing different reordering methods to alter the vertex processing order yielded varying numbers of iterations and runtimes. % when executing the PageRank algorithm on the reordered datasets. 
% An explanatory instance of this phenomenon is depicted in Figure \ref{fig:reorder-direct}. \gsf{see comment} %重新画这个图，一眼就能看出不同的order，收敛速度不同。不要牵扯message，别人不知道为啥会有message，message只有在顶点为中心或者分布式的情况下才有，这里只说顶点状态就行。
% It can be seen that the processing order <d, c, b, a>
%可以看出
%这是因为在处理b时用到了顶点a本轮迭代后的最新状态，而order2中处理顶点b时用的是顶点a的上一轮迭代状态。用最新的状态往往更容易使顶点达到收敛状态。
%An explanatory example of this phenomenon is illustrated in 
% \eat{Figure \ref{fig:pr-eg-2} and Figure \ref{fig:pr-eg-3} list the states (PageRank values) of vertices after the first three iterations \zyj{and the total rounds of iteration} for different processing orders.}
Initially, all vertices have the same PageRank value of 0.25. The \textit{Vertex Processing Order 2}, $d-c-b-a$, makes the vertices states change faster, resulting in fewer iterations (only 26). Since $c$, $b$, and $a$ are updated using the latest state values of vertices $d$, $c$, and $b$ that are updated just now in the current iteration. While according to \textit{Vertex Processing Order 1}, 
to update the vertices $c$, $b$, and $a$, we use the values of $d$, $c$, and $b$, respectively, which are updated in the previous iteration.
% vertices $c$, $b$ and $a$ are updated using the values of $d$, $c$ and $b$ that are updated in the previous iteration. 
Performing computations based on the latest state values of neighboring vertices usually makes it easier for the vertices to reach the converged state\cite{zhang2011priter, zhang2013maiter}. 
% \eat{Therefore, if the vertices can be reordered and stored in the order of processing, the updated state of the previous vertices can be used by the latter vertices in the current round of iteration, thus speeding up the iteration.} 
A question naturally arises, \textit{how can we obtain a better vertex processing order that accelerates the change of vertices state?} %tables represent the state values of each vertex after each step of the first iteration. It can be observed that when the processing order is $a$-$b$-$c$-$d$, except for vertex $d$, all other vertices can only use their current state values. However, when the processing order is $a$-$d$-$c$-$b$, the vertices at the back of the processing queue can utilize the latest state values of the vertices in front of them. Computing based on the latest state values often makes it easier for the vertices to reach the convergence state.
% When the message passing direction is $a\rightarrow b\rightarrow c$, it aligns perfectly with the vertex processing order. Thus, upon $a$ updating its state, $b$ immediately utilizes the latest state of $a$, and so can $c$. However, when the message transmission direction is opposite to the vertex processing order, $a$ updates its state but cannot instantaneously relay it to $c$. It can be inferred that organizing data in the processing order enables sequential reading of graph data, leading to improved performance in graph processing.

% \begin{figure}[t]
% \centering
% % \captionsetup{justification=centering}
% \includegraphics[width=0.95\linewidth]{Figures/simple.png}
% \caption{The impact of different message processing order on iteration performance.}
% \label{fig:reorder-direct}
% \end{figure}



%在处理顶点时往往按照在内存中的顺序来处理，这样可以顺序访问内存中需要处理的点，提高cpu的cache命中率，减少cache和memory之间io的开销。因此需要按照处理顺序对图数据进行reorder。但是即使顺序更新顶点，仍然会有大量的io\cite{zhang2016optimizing，sigmod那个}.因为处理每个顶点时会访问或者更新其邻居的状态，这会导致大量的random access。Zhang等人\cite{zhang2016optimizing}调研了图处理系统会有60-80%的开销在cache和memory之间的io上。当前也有一些提升io的工作，但是他们忽略了顶点更新顺序带来的收益。如何在不提升cache与memory之间io的前提下，找到一个较好的处理顺序？这给图处理顺序的寻找增加了难度。一种既需要考虑顶点处理顺序，又考虑cache命中率的方法需要提出。\del{在处理每个顶点时要读取或更新邻居顶点的状态。为了能够提高局部性，往往顶点的邻居与顶点在内存中放在一起，提高cache命中率。，此外，更新完自己后，更新邻居，也会带来较好的因此迭代计算时顶点更新时会读取或频繁读取和更新顶点的状态，如果顶点的邻居在处理图数据时，我们往往按照顶点的排列顺序进行处理，这样可以按顺序读取和写入数据。按处理顺序对数据进行排列，可以按顺序读取图数据，从而提升图处理性能。这需要对图数据进行重编号。即使按顺序既顶点id递增连续处理图数据，仍然会有内存，研究表明会有60-80%的开销在cpu和memory之间的IO\cite{}。这主要是因为顶点需要访问邻居，邻居不挨着，频繁random access，而邻居挨着，则会提高cache命中率。因此，在reorder时不仅要考虑顶点更新效率，而且要考虑顶点之间的局部性。如何在保证更新效率的同时，做到局部性？}
% \zyj{However, it is not feasible to pursue the perfect consistency between the order of vertex updating and vertex processing, that is, like processing order 2, each vertex can iterate based on the latest updated vertex state of its neighbors.}
\stitle{Observation 2.} During the iterative computation of graphs, the processing of vertices typically follows the order in which they are stored in memory. This sequential approach enables efficient access to the vertices in  memory for processing, since it improves CPU cache hit rate and mitigates I/O overhead between cache and memory.
% This sequential approach enables efficient access to the vertices that require processing in memory, since it improves CPU cache hit rates and mitigates I/O overhead between cache and memory. 
% \yaof{yao:"that require processing in memory" which is ambiguity, it is not processed in memory, it is a memory access problem. Another version: This sequential approach enables efficient access to the vertices in  memory for processing, since it improves CPU cache hit rates and mitigates I/O overhead between cache and memory. }
% \eat{Therefore, the vertices should be reordered in accordance with the processing order.}
% \zyj{Hence it will be beneficial if the vertices are reordered in the order of processing.} 
% \yaof{yao: what does the above sentence mean?}
However, even processing vertices in the order of their storage in memory, 
% \eat{However, it is not feasible to arrange vertices completely according to their processing order.} 
significant I/O overhead may still arise when accessing or updating the state of neighboring vertices, particularly when these neighbors are spatially distant
% during the vertex processing phase
\cite{zhang2016optimizing,wei2016gorder}.
% if the neighbors are far away from each other during vertex processing 
%This is due to the interrelated complexity of graph data, which can result in significant random access overhead.一味追求减少迭代次数的order可能会破坏原始图数据的局部性，而导致io开销变大。
Only pursuing the processing order
% that can 
to minimize the number of iterations may destroy the locality of the original graph, which may result in greater I/O overhead between the CPU cache and main memory.
% 将顶点仅按照处理顺序进行排列而不考虑其他因素，表1展示了在不同数据集上如此排序后与原始图的对比结果。虽然排序后的迭代轮数都减少了，但是cache miss数量却增加了。这是因为破坏了图的局部性，导致cache命中率下降。
% 怎么排序的不用说

Table \ref{tab:factor} shows %the comparative results between 
the number of iterations and the total number of cache misses when performing PageRank on the original graph and a reordered graph %. the original graph and the reordered graph 
% reordered graph and the  
across different datasets. 
% The vertices on the reordered graph are arranged solely based on their processing order without considering other factors. 
Obviously, \eat{while}although the number of iterations required to reach the converged state decreases after reordering, there is an increase in cache misses. We find that the graph reordering may disrupt the locality of the original graph where the vertices and their neighbors are far away from each other %This is attributed to the disruption of graph locality, 
which results in a decline in the cache hit rate.
% \gsf{show a table to motivate the I/O and exaplain it}\eat{Zhang et al.\cite{zhang2016optimizing} have reported that 60\%-80\% of the overhead in graph processing systems is attributed to the I/O between CPU cache and main memory.} 
% Taking into account the IO communication between the CPU cache and main memory makes it more difficult to find an optimal graph processing order. While some efforts have been made to improve I/O performance \cite{}, \gsf{they did not take into account the update rate of vertices state. %the benefits of vertex update order}%应该是他们只关注减少io，而忽略了顶点更新速度，
%On the other hand, 
Accounting for I/O communication between the CPU cache and main memory adds complexity to finding an optimal processing order.
Some attempts have been made to enhance I/O performance \cite{arai2016rabbit,wei2016gorder}, but they have not taken into consideration the acceleration of the vertices' state change.
% \zyj{There are many studies on improving I/O performance\cite{arai2016rabbit,wei2016gorder}, but there is little research that has considered the issue of accelerating the vertices' state change.}
%The question remains: 
\textit{How to identify an optimal processing order that enables vertices to be updated faster without compromising I/O communication between the CPU cache and main memory?} %The search for an optimal graph processing order poses a significant challenge. To address this challenge, a method that takes into account both the vertex processing order and cache hit rate needs to be developed.
% The distribution of vertices in natural graphs is often imbalanced, resulting in a non-consecutive alignment of adjacent vertices in memory and random data access. According to experiments reported in \cite{zhang2016optimizing}, the memory stalls caused by the cache misses account for 60\%-80\% of the total graph computation time. Based on the continuity of graph data access, it is desirable to have a vertex's neighbors arranged as closely as possible to improve the cache hit rate. Therefore, when reordering, it is necessary to consider not only the processing order and update efficiency of vertices but also the locality between vertices.

%challenge:In summary，解决上述问题需要解决两个问题，一个是order好坏的衡量，虽然可以通过迭代次数来衡量一个order的好坏，但在我们未执行图分析算法之前不知道order的好坏，即order好坏的衡量没有标准，因此在寻找一个好的order之前需要寻找一个衡量order好坏的衡量标准，which是非常困难的。Furthermore，processing order中顶点状态变化快与局部性之间的co-design。
% challenge1：如何决定order
% challenge2：co-design take into consideration both the the rate of vertex state change and locality

% In summary, solving the above problems requires addressing two challenges

\stitle{Challenges.} In summary, solving the above problems requires addressing the following two challenges. \romannumeral 1) How to measure the effectiveness of the graph processing order before performing iterative computation. While the number of iterations can serve as a metric, evaluating the quality of processing order before executing the graph analysis algorithm poses a challenge. \romannumeral 2) There is a co-design issue in finding a graph reordering method that both considers the rate of vertex state change and the locality of vertices and their neighbors when processing graphs.


%为了衡量processing order，我们提出了latency distance.它描述了更新顶点时多少邻居的状态在当前迭代中还未被更新。基于obseravation1的分析，在更新顶点时，如果其邻居顶点已经在当前迭代中更新，则使顶点的状态变化更大。因此在更新每个顶点时，我们应该使尽量多的邻居已经被更新。既latency distance更细小。我们应该减少还未更新邻居的数量,降低latency distance的值，既，而是尽可能多的邻居已经更新。我们从以顶点为中心的消息传播角度解释了latency distance来衡量order加速顶点变化的合理性（第3.1）。为了既减少latency distance又保证每个顶点与其邻居在processing order中的局部性，我们提出来GoGraph图重排序算法。该算法尝试将出度大，入度小的顶点放在order的前面，而出度小入读大的放在order的后边。同时，为了保证局部性，在每个顶点的出邻居尽量放在每个顶点的后边。
\stitle{Our Solution.} To evaluate the effectiveness of graph processing order in accelerating the vertex changes before iterative computations, we propose %a metric called 
\emph{Latency Distance}.
%to evaluate the quality of the specified processing order of graph vertices and thus obtain a judgment on the efficiency of the iterative computation before the graph algorithms run. 
It describes the number of neighbors, which have not been updated in the current iteration, used when processing vertices.  %messages passed by vertices in the same iteration that are not utilized for updating the state values of subsequent vertices under the graph topology. 
Based on the analysis in Observation 1, when updating a vertex, its state will change more if its neighbors have already been updated in the current iteration. Therefore, when processing each vertex, it is better to ensure as many neighbors as possible have been updated. Put differently, when processing vertices, we should reduce the number of neighbors that have not been updated, i.e., minimize the latency distance. Therefore, latency distance can be used as a metric to measure the effectiveness of processing order in accelerating vertex changes.
To minimize the latency distance of processing order while ensuring the locality of vertices and their neighbors, we propose a graph reordering method, GoGraph. It tries to put vertices with large out-degree and small in-degree at the front of the processing order, and vertices with small out-degree and large in-degree at the end of the processing order.%因为
\eat{By reordering the vertices in a manner  that maximizes the utilization of messages in the same iteration, we can effectively minimize the latency distance, which facilitates faster propagation of
vertex state values, resulting in faster changes in each iteration and approaching the converged state. 
Therefore, based on the guidance of latency distance, we propose a graph reordering method, \go.} 



%\stitle{Challenge I.} How to find a proper order 

%\stitle{Challenge II.} In summary, solving the above problems requires addressing two challenges.

% \stitle{Challenge II}
% \zyj{Solving the above-mentioned issues requires addressing two challenges. One of the primary concerns is determining the quality of vertex ordering. While the number of iterations can serve as a metric, evaluating the quality of ordering before executing the graph analysis algorithm poses a challenge. Consequently, finding a reliable measure of ordering quality prior to the search for optimal ordering becomes a demanding task. Furthermore, there is a co-design issue between the rapid changes in vertex state and locality in the processing order.}

%为解决上述问题，本文提出了一种graph reordering algorithm，GoGraph，其在对顶点进行重排序时综合考虑的顶点的更新顺序和顶点的局部性。GoGraph利用了图计算中顶点为中心的模型，其中顶点的更新被抽象成顶点之间消息的传播。我们发现在以顶点为中心的模型中，利用最新的更新的本质是消息的传播距离短速度快。基于此，我们提出了latency distance的概念。latency distance来衡量顶点状态的传播速度。用latency distance来指导寻找顶点的处理顺序，最小化latency distance就是一个好的processing order。而为了保持局部性，在进行reorder的时候，考虑了顶点的邻居，即尽量将同一个顶点的所有邻居放在一起，这是一个简单但是实用的方案。
% 【对于分布式的场景，在某个partition中，会有一些点没有出度（mirror点？）或有一些点没有入度（什么点？），针对此问题，我们提出了分布式场景下的reorder方法。】--->【对于分布式场景，不同机器上的边界点在参与了本机上的迭代后，还需要与其他机器进行消息传播，为确定这些顶点的排序位置，我们提出了分布式场景下的reorder方法。】
% ***。\del{基于此提出了GoGraph算法来最小化latency distance简介GoGraph为了能够刻画order的好坏，我们提出了latency distance。latency distance是顶点更新后被邻居利用的距离，如果能立即被邻居利用，即邻居利用率最新的状态，加速顶点状态更新，更快收敛。}
%简单介绍与GoGraph相关的三个贡献，给出intuition，然后summary一下contribution。

% To solve the aforementioned challenges, we\eat{ first} propose the \textit{Latency Distance} to measure the present a graph reordering algorithm named \go, which takes into account both processing order and vertex locality %during the reordering process. 
% when reordering the graphs. %为了衡量processing order的好坏，我们提出了latency distance。迭代计算可以被抽象成顶点之间的消息传播，既以顶点为中心的迭代计算模型\cite{pregel,powerGraph,Maiter，ingress，layph}，which在分布式图计算系统中通常应用。顶点利用接收到的邻居发来的消息更新自己的状态，然后生成消息发送给邻居。
% 【如果一条消息生成之后立即被邻居利用，则说明该消息传播速度非常快。一条消息从生成到邻居利用这条消息进行更新作为消息传播的距离。如果该距离小，则说明消息被立即利用，且被转发出去，消息传播速度快，顶点状态变化就快。如果太远，则消息很久才被利用并转发，消息传播速度变慢，顶点状态变化就慢。传播越快，每个点收到的越多，每次更新顶点状态变化就越大。】【这一段我想改一下，见下面】
%为了最小化latency distance，我们提出了GoGraph。抄abstract里边的gograph的介绍。
%扩展了分布式。
% To evaluate the graph processing order before iterative computation, 
% To evaluate the vertex processing order before the start of iterations,
%In \go, vertex updates are abstracted as the propagation of messages between vertices, adhering to the 

% 为了解决上述挑战，我们提出了一个称为Latency Distance的度量。我们利用了图计算中顶点为中心的模型将顶点的更新抽象成顶点之间消息的传播。它在分布式图计算系统中通常应用。顶点利用接收到的邻居发来的消息更新自己的状态，然后生成消息发送给邻居。随后，对于一条消息从发出到被使用的时间上的间距，我们将它抽象为具体的距离，也就是latency distance。
\eat{To solve the aforementioned challenges, we propose a metric called \textit{Latency Distance}. We use the vertex-centric graph processing model to abstract the update of vertices into the propagation of messages between vertices. It is applied widely in graph processing systems\cite{malewicz2010pregel, gonzalez2012powergraph, zhang2013maiter, gong2021automating, yu2023layph}, where vertices use the messages received from their neighbors to update their state, and then generate messages to be sent to their neighbors. Afterwards, we abstract the time interval from sending a message to its usage into a specific distance, i.e., latency distance.}
% The iterative graph computation can be abstracted as messages passing between vertices, known as the %i.e., %In the 
% vertex-centric graph processing model, which is applied widely in graph processing systems \cite{malewicz2010pregel, gonzalez2012powergraph, zhang2013maiter, gong2021automating, yu2023layph}. In the vertex-centric model, vertices use the messages received from their neighbors to update their state, and then generate messages to be sent to their neighbors. 
% If a message is used immediately after it is generated, it means that the message spreads very fast. Latency distance is the distance of message propagation, that is, the number of vertices processed between message generation and consumption. The smaller the latency distance means that the message is used immediately, that is, the message spreads faster. The vertex state changes faster, and vice versa. 
% 【如果在一轮迭代中，一个顶点发出的消息在传递给后继的顶点之后，后者在进行状态值的更新时用上了这条消息，就说这一条消息在本轮中得到了使用。否则，只能在下一轮中得到使用。因此我们使用latency distance对一个顶点传出的消息使用的时间进行量化。如果能在本轮中被使用，latency distance就是0，否则就是1。如果能通过重排序的操作使得每个顶点传出的消息都能被后继顶点在本轮中得到使用，即尽可能减少latency distance的值，按照我们之前的分析，这将有利于顶点状态更快的传播，在每轮迭代中顶点状态的变化就会更快，每一轮迭代的结果接近于收敛时的状态值。】
\zyj{A message delivered from a vertex is defined as being \textit{utilized} in the current round if it takes effect in updating the state value of a subsequent vertex. Otherwise, the message can only be utilized in the subsequent round. Therefore, latency distance can be used to represent the time interval between the transmission and utilization of a message. If a message can be utilized within the same iteration, its latency distance is 0; otherwise, it is 1. By reordering the vertices in a manner that maximizes the utilization of messages within the same iteration\eat{ by its succeeding vertices}, we can effectively minimize the latency distance. As discussed earlier, this facilitates faster propagation of vertex state values, leading to faster changes in each iteration and approaching the converged state.}
% latency distance能够衡量消息传播速度。一个processing order的传播速度越快说明processing order越好。因此latency distance能够衡量processing order的好坏。利用latency distance来衡量order的好坏，就变成了最小化latency distance。
% Therefore, latency distance can measure the effectiveness of the processing order. Then, finding a vertex processing order that minimizes that number of iterations becomes finding a processing order that minimizes the latency distance.
% Therefore, latency distance serves as a metric to evaluate the efficiency of the processing order. 
Thus, finding a vertex processing order that minimizes the number of iterations is equivalent to finding a processing order that minimizes the latency distance.

%The fast spread of the message is conducive to the rapid change of the vertex state. %vertices updates are abstracted as the propagation of messages between vertices. A message from generated to We discover that the essence of utilizing the latest updated state of neighboring vertices is minimizing the distance between two vertices and optimizing the speed of message propagation. %To evaluate the propagation speed of the vertex state, we introduce a metric called \textit{Latency Distance}, which measures the storage separation between a vertex and its neighboring vertices. 

%基于latency distance，我们设计了gograph。在进行reorder的时候，我们综合考虑了消息的latency distance和顶点之间的局部性，将顶点的邻居放置在其后边
We further propose a graph reordering method, GoGraph. 
% GoGraph tries to insert the high outdegree vertex’s outgoing neighbors behind and closer to it and puts outgoing neighbors of the same vertex together. 
\zyj{To reduce latency distance, we place vertices with high out-degree towards the front of the processing queue. Since the vertex with high out-degree will propagate messages to many out-neighbors, resulting in a latency distance of 0 between the vertex and its out-neighbors. Similarly, the vertices with high in-degree are placed towards the back of the processing queue. Besides, to maintain locality, we put the neighbors of a vertex together.}
In this way, GoGraph not only improves the efficiency of message passing but also reduces the number of CPU cache misses. Furthermore, we also implement GoGraph into the distributed graph processing systems to improve their performance.
%Utilizing this metric as a guiding principle, we can discern an optimal vertex processing order, where the sequence of vertices that minimizes latency distance serves as an indicator of superior processing efficiency. In terms of preserving locality, adequate consideration is given to the neighboring vertices of a given vertex. Our objective is to maximize the grouping of neighbors belonging to the same vertex. This approach represents a straightforward yet effective solution. For distributed scenarios,  boundary vertices on different machines are involved in local iterations and subsequently require message propagation across machines. We propose a reordering method specifically designed for distributed environments, which aims to determine the appropriate position for these vertices within the distributed context.


% leverages the sequential nature of message propagation and the utilization of the latest states in asynchronous systems for iterative computations. The objective is to perform vertex reordering to achieve a consistent alignment between the processing order of vertices and the order of message utilization, while also enhancing the locality of vertex neighbors as much as possible. To evaluate the compatibility between the order of vertex processing and message utilization, we introduce a metric called \textit{Latency Distance}. This metric measures the distance between a vertex and its neighbor in terms of message utilization efficiency. Specifically, if a neighbor vertex can immediately utilize a message passed by the sender vertex within the current iteration, their distance is deemed to be $0$, otherwise, it is incremented by $1$. Based on the \textit{Latency Distance} concept, \go prioritizes placing vertices that send out many messages towards the front of the sequence and those that receive many messages towards the back. This ordering ensures that receiving vertices can make the most of the incoming messages, allowing for effective message utilization during a single iteration.

% To enhance the efficiency and scalability of our proposed reordering algorithm for large-scale graphs, we adopt a distributed approach. The first step is to partition the graph into clusters and distribute them across multiple nodes. For clustering, we leverage the incremental aggregation method\cite{arai2016rabbit} to improve the modularity of the graph. The vertices within each cluster are divided into internal and external vertices based on whether they exchange information with the vertices in other subgraphs. For internal vertices, we employ the same reordering algorithm as on a single machine. For external vertices, we divide them into entrance vertices and exit vertices. Entrance vertices need to receive messages from other nodes, and therefore require the highest priority, ensuring that the messages sent by external vertices are efficiently utilized by the internal ones.

% Last but not least, we conduct experiments to compare the performance of \go with other state-of-the-art reordering algorithms on various real-world graphs. The experimental results demonstrate that \go can significantly reduce the convergence time of iterative computation by enhancing the efficiency of message passing and minimizing the number of cache misses. \zyf{this contribution seems weak. }


%Contribution of the paper
\stitle{Contributions.}
The contributions of our study can be summarized as follows:

\begin{enumerate}[label=\arabic*.]
% \item We propose an innovative approach that considers the direction of message propagation in iterative computing and integrates it with the vertex processing order to optimize the message utilization within a single iteration. \zyf{does this overlap with the second one? Is the metric latency distance sufficient to be considered as a contribution? may need some analysis or proof.}
% \item Our proposed method, GoGraph, considers both the message send and receive behavior of vertices and incorporates locality considerations. By optimizing message utilization and minimizing cache evictions, our approach enhances the performance of iterative computations.
% 贡献1：latency distance
\item This paper 
% introduces a vertex reordering algorithm called \go. It 
innovatively proposes the concept of Latency Distance, which quantifies the quality of the ordering by calculating the spatial distance between vertices.
% 贡献2：distance和cache的关系。我们研究了顶点处理和IO访存的关系，在保证图处理顺序与顶点存储顺序一致的基础上，我们还考虑了图的局部性，以减少cache miss，提高迭代效率。
\item We investigate the relationship between vertex processing and I/O access. Our reordering method minimize the latency distance under the premise of ensuring graph locality.
% encompasses not only preserving the consistency between the graph processing order and the vertex storage order but also incorporating graph locality to minimize cache misses and thereby enhance the efficiency of iterative computations.

% 扩展到分布式时 对每个分区都可以reorder
\item We adopt effective strategies for graph partitioning and deployment to different nodes to handle large-scale graphs. We have adopted the \go algorithm into a distributed version, where reordering is performed on each node to enhance iterative computation efficiency and inter-node communication efficiency.
% \item We conduct extensive experiments to validate the effectiveness of our proposed reordering method in promoting message passing and reducing cache misses, thereby improving iteration efficiency. Our results confirm the effectiveness of the \go algorithm. \zyf{this is weak.}
\end{enumerate}





%后边说图处理分两步，一个是内部便利，一个是机器之间协作。我们优化内部便利效率。
% To optimize graph processing efficiency, there are two main steps: optimizing the traversal order within a single node and optimizing collaboration between different machines. The focus of this paper is on improving internal traversal efficiency. 
The structure of this paper is as follows. Section \ref{sec:pre} provides an overview of the background and notations related to iterative computation and graph reordering. Section \ref{sec:method} presents our proposed reordering method, first introducing the approach under single-machine conditions, and then elaborating on the method under distributed conditions. Section \ref{sec:expr} presents various experiments and detailed experimental results. Section \ref{sec:relate} introduces the related work. Finally, we conclude our paper in Section \ref{sec:conclu}.
% Iterative graph computation includes local computation within each individual vertices and message passing between vertices, can become computationally intensive when analyzing large-scale graphs due to the repeated access and computation of vertices and message passing along edges until the graph converges.

%To address the efficiency problem of graph analysis, many studies have focused on optimizing the iteration process. For example, in \cite{zhang2013maiter}, each vertex buffers the state changes incrementally, propagating the accumulated value to the neighbor vertices only after it reaches a preset threshold. This method improves computation efficiency by reducing the number of address lookups, thereby reducing the chance of cache misses.
%Another popular approach is to reorder the vertices to improve graph locality. This method stores the vertices that will be accessed successively in time or space together, swapping them into the cache simultaneously \cite{zhang2016optimizing,arai2016rabbit,wei2016gorder}. This technique improves addressing efficiency and reduces memory replacement times.



% \begin{table}
%     \centering
%     \caption{The Effect of different reordering methods on \protect\\ distance and number of iterations}
%     \vspace{-2mm}
%     \label{table:table1}
%     \begin{tabular}{ccccc}		
%         \toprule
%          & & Origin & Deg Sort & Gorder\cite{wei2016gorder} \\
%         \midrule
%         \multirow{2}*{Stanford} & Iter Rounds & 67 & 74 & 73 \\
%             ~ & Latency & 75,806,815  & 139,828,032  & 130,099,724 \\
%         \midrule
%         \multirow{2}*{Berkstan} & Iter Rounds & 67 & 77 & 76 \\
%             ~  & Latency & 164,387,256 & 281,283,590 & 302,202,240 \\
%         \midrule
%         \multirow{2}*{Google} & Iter Rounds & 66 & 70 & 80  \\
%             ~ & Latency & 164,387,256 & 281,283,590 & 302,202,240 \\
%         \bottomrule
%     \end{tabular}
%     \vspace{-5mm}
% \end{table}


% The total overhead of graph iteration is determined by the number of iteration rounds and the expense per round. Previous methods have focused on reducing the memory stall overhead per round by improving cache hit rates or reducing cache replacement costs. However, these methods may increase the iteration rounds because the amount of message propagation per round decreases, while the total amount of messages modified towards convergence remains constant.
% Prior research did not address iteration reduction as an optimization objective, but we believe it is crucial. Since each iteration of a large graph involves processing numerous vertices, reducing the number of iteration rounds can significantly minimize the total cost.
% Prior research has not considered reducing the number of iterations as a primary optimization objective. Nonetheless, given that each iteration of large-scale graphs involves processing multiple vertices, minimizing the number of iterations can have a significant impact on reducing the overall computational cost.
% Table \ref{tab:nd-it} displays the number of iterations required for PageRank to converge on different graph datasets, which are reordered with different methods. Although many reordering algorithms claim to enhance the efficiency of graph computation, they may also lead to an increase in the number of iterations, which in turn can impact the overall performance. If the number of iterations can be minimized during the reordering process, the performance of graph computation could be significantly enhanced.

% Reducing the number of iterations required for graph computation is crucial to improve its overall efficiency. The key lies in maximizing the information utilized and transmitted per iteration. 
% The key of reducing the number of iterations lies in maximizing the information utilized and transmitted per iteration.
% Message passing is the prevalent technique for iterative computation in most graph processing systems, whereby each vertex transmits messages to its out-neighbors, which then update their states based on the received information. The messages represent the state changes and are progressively reduced until the convergence threshold is reached. By optimizing the content and routing of these messages, it is possible to reduce the total number of iterations required to achieve convergence.

% Many studies have focused on vertex reordering to improve graph locality. For example, Rabbit Order\cite{arai2016rabbit} reorders vertices based on the hierarchical community structures, such that frequently accessed vertex communities are mapped closer to the CPU cache hierarchy, and vertices in the same hierarchy are co-located. Another example is Gorder\cite{wei2016gorder}, which reorders vertices based on their intimacy, arranging vertices with more shared parents or siblings together. While these methods effectively improve locality, they do not account for the order of message delivery. FBSGraph\cite{fbsgraph}, on the other hand, considers the cascade effect between vertices and partitions the graph into paths based on message-passing routes to accelerate the propagation of state changes. This approach takes into account the sequential nature of state changes that might affect subsequent vertices. Nevertheless, FBSGraph's reliance on the DFS algorithm for path exploration may render its partitioning of high-degree vertices unreasonable, thereby potentially hindering the propagation of messages.

% The proposed reordering algorithm in this paper, \go, 


